On the role of population heterogeneity in emergent communication

Populations have often been perceived as a structuring component for language to emerge and evolve: the larger the population, the more structured the language. While this observation is widespread in the sociolinguistic literature, it has not been consistently reproduced in computer simulations with neural agents. In this paper, we thus aim to clarify this apparent contradiction. We explore emergent language properties by varying agent population size in the speaker-listener Lewis Game. After reproducing the experimental difference, we challenge the simulation assumption that the agent community is homogeneous. We first investigate how speaker-listener asymmetry alters language structure to examine two potential diversity factors: training speed and network capacity. We find out that emergent language properties are only altered by the relative difference of learning speeds between speaker and listener, and not by their absolute values. From then, we leverage this observation to control population heterogeneity without introducing confounding factors. We finally show that introducing such training speed heterogeneities naturally sort out the initial contradiction: larger simulated communities start developing more stable and structured languages.

==> brouillon_related.tex <==
paragraph{Populations in emergent communication.} 
% Intro emecomm
Works in deep emergent communication debate the prerequisites to the emergence of language universals (compositionality~\citep{li2019ease,lazaridou2018emergence,mordatch2018emergence,resnick2019capacity,kottur-etal-2017-natural,choi2018multiagent,Kuciski2020EmergenceOC}, generalisation~\citep{baroni2020,chaabouni2020compositionality,hupkes2020compositionality,denamganai2020emergent}, efficiency~\citep{chaabouni2019anti,rita-etal-2020-lazimpa}, stability~\citep{kharitonov2020entropy}, etc.) mainly through the study of inductive biases and cultural transmission. 

% Transition sur les populations
Recent works have started exploring the impact of population structures on deep emergent languages. Properties of emergent languages (ie. emergence of common language, compositionality, abstraction, generalization) are often discussed in regard of the community size.
% common language
Indeed \citet{harding-graesser-etal-2019-emergent} shows, as part of a contact linguistics study~\citep{myers2002contact}, that speakers start to develop a common language as soon as populations are composed of at least 3 agents (represented as both speakers and listeners). This result shows that speakers' coordination can be obtained without the introduction of an innate mechanism that ties speaking and listening such as an obverter technic~\citep{choi2018multiagent} or theory of mind~\citep{Zhu2021}.  \citet{bouchacourt-baroni-2019-miss} completed this result by studying full-symmetry between agents. They show that full-symmetry is not a sufficient condition to the emergence of a common language and also suggest that languages should diffuse in larger communities in order to synchronize. Population size can therefore be a necessary and sufficient condition to the emergence of a common language within a community of speaker.
%other properties 
Additionally, early results show that other language properties are affected by population size. While studying cultural transmission, \citet{cogswell2020emergence} exhibit a slight compositionality enhancement when increasing population size without the need of language transmission. Analogously, \citet{tieleman2019shaping} explicitly studies community size and display a small but consistent gain of abstraction and structure within speakers' latent representations by increasing population size. Eventually, \citet{fitzgerald2019populate} shows that populations improve regularization and generalization compared to single speaker-listener pairs but underlines that there is not a clear correlation between community size and leaning properties.
% IN this paper
In this paper, we will start by studying the impact of community size. We will show in the context of reconstruction games that population size indirectly affects the learning dynamic but is actually not a structuring factor per se. In particular, we will show that population effects can be reproduced with a single speaker-listener pair and even canceled when playing with other factors.




%% Old version


Studying population structures start to flourish. The first fundamental question asked is which conditions several (2 and more) agents adopt a common language protocol ? First approach~\citep{choi2018multiagent} introduced a direct transfert between listening and speaking modalities via an obverter technic~\citep{oliphant1997} \mathieu{à vérifier que ça touche bien la question du langage commun}, explicitly forcing speakers coordination. Conversely, it has been demonstrated that increasing population size can indirectly help to coordinate agent without the need of an innate mechanism that ties listening and speaking. Indeed \citet{harding-graesser-etal-2019-emergent} shows, as part of a contact linguistics study~\citep{myers2002contact}, that common language can emerge indirectly and states that the only required condition is a minimal number of agents within the population (3 agents represented as both speakers and listeners). This result is completed by \citet{bouchacourt-baroni-2019-miss} who study full-symmetry between agents. They show that full-symmetry is not a sufficient condition and also suggest that languages require diffusion in larger communities in order to coordinate. Other early results exhibit an improvement of language properties by increasing community size. While studying cultural transmission, \citet{cogswell2020emergence} show that increasing population size enhance compositionality without the need of language transmission. Analogously, \citet{tieleman2019shaping} explicitly studies community size and display a gain of abstraction and structure within speakers' latent representations by increasing population size. Eventually, \citet{fitzgerald2019populate} shows that populations improve regularization and generalization compared to 2 agents systems but underlines that there is not a clear correlation between community size and leaning properties. In this paper, we will start by studying the impact of community size. We will show that in the context of reconstruction games, population size indirectly affects the learning dynamic but is actually not a key factor per se. In particular, we will show that population effects can be reduced to 2 agents settings by playing with the learning speed asymmetry between speakers and listeners.




\subsection{Language regularization is better explained by the ratio between the number of speakers and listeners than the community size}

As discussed in the related section, community size may enhance language properties when being sufficiently large~\cite{choi2018multiagent,harding-graesser-etal-2019-emergent,tieleman2019shaping,fitzgerald2019populate}. In this section, we observe that the total number of agents have little impact. Instead, we show that the ratio between the number of speakers and listeners effects language properties. We then explore whether the population asymmetry could be a compounding factor of a deeper process. Finally, we hypothesis that the core phenomenon is a learning dynamics, or learning speed, which is triggered by such asymmetry. 

\paragraph{Speakers/listeners asymmetry better effects language properties than raw population size} In Figure \ref{fig:prop_f_steps}, \mathieu{expe en cours}, we first assess \mathieu{directement: observe} whether the community size is correlated with emergent languages properties enhancement (entropy, generalization, robustness to noise, compositionality). As shown in \mathieu{???} where we measure those properties while increasing the community size (with $N_{speakers}=N_{listeners}$), \textit{blablabla}. However, we observe on \mathieu{Fig ??}, that increasing $N_{listeners}$ when $N_{speakers}$ is fixed tends to improve emergent languages structures (lower entropy, better compositionality) and communication performances (better robustness and generalization). 
On the contrary, the language structure impoverish when increasing $N_{speakers}$ while keeping $N_{listeners}$ constant, e.g, poorer structures (higher entropy, worse compositionality) and worse communication performances (lack of robustness to noise and low test-accuracy). 
In a few words, the more speaker there are regarding the number of speaker, the better is the language.


However, we observe on \mathieu{Fig ??}, that increasing $N_{listeners}$ when $N_{speakers}$ is fixed tends to improve emergent languages structures (lower entropy, better compositionality) and communication performances (better robustness and generalization). 

On the contrary, the language structure impoverish when increasing $N_{speakers}$ while keeping $N_{listeners}$ constant, e.g, poorer structures (higher entropy, worse compositionality) and worse communication performances (lack of robustness to noise and low test-accuracy). 



\paragraph{The asymmetry between the number of speakers and listeners control language properties} Based on these observations, we introduce the ratio $\rho_{num /agents}:=\frac{N_{listeners}}{N_{speakers}}$ that controls the relative number of listeners and speakers within the community. On Figure \ref{fig:prop_f_splist}, we observe a strong impact of $\rho_{num /agents}$ on the entropy. When, $\rho_{num /agents}$ is very low, speakers tend to produce languages of very high entropy, meaning that they use a large number of different messages to refer to a same meaning $x \in \mathcal{X}$ ($\pi_{S}(m|x)$ is flat). On the contrary, for large values of $\rho_{num /agents}$, Speaker's policies have a very low entropy meaning that agents almost use a unique message by concept $x$ (almost a 1:1 mapping).

\paragraph{Population effect or learning asymmetry between speakers and listeners ?} Previous observations raise the question: can population be considered as a regularization factor ? We argue that here population indirectly modify the optimization protocol. Indeed, the number of agents impact the degree of learning of each agent. Since the system is optimized by sampling 1 speaker and 1 listener at each step, each speaker (resp. listener) has a probability $\frac{1}{N_{speakers}}$ (resp. $\frac{1}{N_{listeners}}$) to be drawn. Consequently, each speaker has $\frac{N_{listeners}}{N_{speakers}}$ more or less optimization steps than each listener.

\subsection{Rescaling community effects by playing with learning asymmetry between speakers and listeners}

\paragraph{Controlling learning asymmetry between speakers and listeners} In previous section, we made the assumption that communication properties in community of agents can be improved by increasing the ratio $\frac{N_{listeners}}{N_{speakers}}$ because it indirectly affects the learning protocol. This last hypothesis supposes that we can control languages properties independently of the community size by controlling the learning asymmetry between speakers and listeners. Therefore, we now test whether communication properties can be controlled in a 1 speaker - 1 listener setting by controlling the learning asymmetry between agents. We introduce $\rho_{agents/steps}:=\frac{N_{speaker/steps}}{N_{listener/steps}}$ that measures the ratio of learning steps between the speaker and the listener at each training episode (if $\rho_{agents/steps}=10$, the speaker has 10 times more optimization steps than the listener at each training episode). In particular, if $\rho_{agents/steps}$ is very large (resp. low), the speaker (resp. listener) is almost optimal with respect to the listener (resp. speaker) for every listener's optimization steps (resp. speaker's optimization steps).

\paragraph{Communication properties can be controlled with $\rho_{agents/steps}$}. In Figure \ref{fig:prop_f_steps}, we show the evolution of languages properties as a function of $\rho_{agents/steps}$. On Figure \ref{fig:ent_f_steps}, we note that entropy of emergent languages after convergence continuously evolve with $\rho_{agents/steps}$ between two extreme cases: when $\rho_{agents/steps}$ is very large, the Speaker tends to produce a language of very low entropy ; on the contrary, when $\rho_{agents/steps}$ is very low, the Listener develops high entropy languages. Obtaining low entropy languages is correlated with a gain of compositionality (Figure \ref{fig:compo_f_steps}), generalization (Figure \ref{fig:tacc_f_steps}) and robustness to noise (Figure \ref{fig:noise_f_steps}). \mathieu{plot avec courbes translatées ?}

Results on entropy can be interpreted this way: when $\rho_{agents/steps}\ll1$, speaker is almost frozen from listener's point of view. Therefore, it leaves time for the listener to learn all the messages used by speaker even when speaker's policy is very flat (lots of synonyms). Therefore, as soon as speaker language makes the task feasible \mathieu{pb de mot} (that is there is at least one distinct message referring to each concept), listener stops the training by learning all messages sent by speaker, such that the language has a large entropy (lots of synonyms). On the contrary, when $\rho_{agents/steps}\gg1$, listener is almost frozen from speaker's point of view, meaning that speaker has a very accurate estimation of the reward landscape at every iteration. It then makes it easy for the speaker to target the small set of messages that provide the best rewards (ie. best listener's comprehension). If Speaker's resolution of reward is precise enough (which is the case with a continuous reward), the set of messages providing the best rewards is small enough to converge toward a language of very low entropy (almost a 1 concept : 1 message mapping).

\paragraph{Emergent languages properties are determined by speaker/listener relative learning speed} We have just shown that playing with the relative number of learning steps between agents allow to control emergent languages properties. Actually, the phenomenon at play seems more general: each agent task is characterized by a learning speed and the emergent languages properties are determined by speaker/listener relative learning speed. In order to test this hypothesis, we exhibit two parameters that have a direct impact on the learning speed\footnote{as we study co-adaptive system, it is impossible to have a direct measure of the learning speed}: agents' hidden size and agents learning rates. In Appendix \mathieu{???}, we show how learning speed is influenced by those parameters on static situations. As shown in Figure \mathieu{ajouter les figures}, we see that playing with these parameters (and indirectly the learning speed) produce the same trends we observed with $\rho_{agents/steps}$.

In the end, all experiments simulate situations where the relative learning speed between agents evolves (indirectly by either playing with population properties, optimization or architectural parameters). It is then important to note that phenomena involved in communities of agents can be interpreted with this simple paradigm that applies even at the scale of 2 agents.


==> buffer_3_4.tex <==
% NEW ONE
\subsection{Altering Population Dynamics}
\label{sec:method:heterogeneity}
\vspace{-0.25em}

We now present our method to introduce diversity within a population. We define diversity factors, then propose control parameters to characterize the effects of diversity at the scale of a pair and finally propose a protocol to distribute diversity within a population and thus create heterogeneous populations.

\textbf{Diversity factors}: We aim to vary specific agent features toward creating diversity in the population. In this paper, we specifically target two core components: the training speed and the network capacity. First, we control agents training speed by changing the number of gradient updates. Formally, we introduce the probability $p$ of an agent to be optimized after each iteration of the game. Therefore, the lower $p$, the slower agent training. This approach has two positive features: (i) it neither alters the communication graph nor the agent sampling, preserving other homogeneity hypotheses in the population, (ii) it is more stable than modifying the learning rate as it avoids large destructive updates. Second, we control the network capacity by varying the agent hidden size $h$ in the recurrent core. Note that we only control training speed or network capacity, never both at once. 

\textbf{Control parameters of local asymmetry:} We provide control parameters to characterize diversity at the scale of a pair speaker-listener. Indeed, varying learning speed and agents capacity alters either the absolute and relative learning facilities of agent. To analyze the effect of asymmetrizing a pair of agent, we introduce the relative training speed $\rho_{speed}:=p^{S}/p^{L}$ and the relative capacity $\rho_{capacity}:=h^{S}/h^{L}$ where $p_{S}$ (resp. $p^{L}$) is speaker's learning speed (resp. listener's learning speed) and $h^{S}$ (resp. $h^{L}$) is speaker's hidden size (resp. listener's hidden size).

\textbf{Distributing Population Heterogeneity:} In order to create heterogeneous populations, we propose a protocol to distribute diversity within a population. We characterize every single speaker and listener with individual properties that are sampled once at the beginning of the training. 
%
Formally, when altering training speed, we respectively sample $p_{i}\sim \log\big(-\mathcal{N}(\eta_{p}, \sigma_{p})\big)$
%and $p^{L}_{j}\sim \mathcal{N}(\eta_{p^{L}}, \sigma_{p^{L}})$ f
for every $i$ agent in the population, where $\log\big(\mathcal{N}\big)$ is a log normal distribution. As explained in section~\ref{res:speed}, we only perform this experiment with the update probability factor.


% OLD ONE
\subsection{Altering Population Dynamics}
\label{sec:method:heterogeneity}
\vspace{-0.25em}

\textbf{Controlling factors}: We aim to vary specific agent features toward creating diversity in the population. In this paper, we specifically target two core components: the training speed and the network capacity. First, we control agents training speed by changing the number of gradient updates. Formally, we introduce the probability $p$ of an agent to be optimized after each iteration of the game. Therefore, the lower $p$, the slower agent training. This approach has two positive features: (i) it neither alters the communication graph nor the agent sampling, preserving other homogeneity hypotheses in the population, (ii) it is more stable than modifying the learning rate as it avoids large destructive updates. Second, we control the network capacity by varying the agent hidden size $h$ in the recurrent core. Note that we only control training speed or network capacity, never both at once. 

\textbf{Introducing Population Asymmetry:} In this setting, we break the following population homogeneity hypothesis: `all agents are similar` , and assume that `speaker-listener may be different`. We hence introduce population asymmetry by either altering agent-category training speed or altering the agent-category capacity. 
%
Formally, we define the speaker (resp. listener) training speed $p^{S}$ (resp. $p^{L}$) and hidden size $h^{S}$ (resp. $h^{L}$). To analyze asymmetry at the scale of a pair of agents, we also introduce the relative training speed $\rho_{speed}:=p^{S}/p^{L}$ and the relative capacity $\rho_{capacity}:=h^{S}/h^{L}$ of a pair speaker-listener. Note that we also study the ratio of the number of speakers and listeners in Appendix~\ref{appendix:agents_ratio}, which another diversity factor.

\textbf{Distributing Population Heterogeneity:} In this setting, we break further the population homogeneity hypothesis: `all agents are similar`, and assume that `all agents may be different`. We characterize every single speaker and listener with individual properties that are sampled once at the beginning of the training. 
%
Formally, when altering training speed, we respectively sample $p_{i}\sim \log\big(-\mathcal{N}(\eta_{p}, \sigma_{p})\big)$
%and $p^{L}_{j}\sim \mathcal{N}(\eta_{p^{L}}, \sigma_{p^{L}})$ f
for every $i$ agent in the population, where $\log\big(\mathcal{N}\big)$ is a log normal distribution. As explained in section~\ref{res:speed}, we only perform this experiment with the update probability factor. 
%
%Similarly, when altering network capacity, we respectively sample $h^{S}_{i}\sim \mathcal{N}(\eta_{h^{S}}, \sigma_{h^{S}})$ and $h^{L}_{j}\sim \mathcal{N}(\eta_{h^{L}}, \sigma_{h^{L}})$ for every $i$ speaker and $j$ listener.









Finally, we show that introducing such training speed heterogeneities naturally sort out the initial paradox: larger simulated communities start developing more systematic and structured languages.
%We preliminary explore speaker-listener asymmetry by changing the relative training speed and network capacity, and we observe that it significantly alter language structures. From then, we generate heterogeneous population by modifying the training speed of neural agents. We finally observe that this newly injected heterogeneity naturally sorts out the initial paradox: larger simulated communities start developing more systematic and structured languages. 


%We then analyze other potential sources of heterogeneity and note how they may relate to the training speed, opening for further discussions in AI and sociolinguistics.  
we first explore how speaker-listener asymmetry alters language structure, and find out that 

find out that the relative training speed dynamics controls emergent language properties.

find out that controling the relative training speed dynamics enable to safely inject henteorogenity without confounding factor.

We first explore how speaker-listener asymmetry alter language structure to examine two potential controlling factor: relative training speed and network capacity. From then, we manage to robustly control population heterogeneity without introducing confounding factors. Finally, we show that introducing such heterogeneities naturally sort out the initial paradox for larger communities start developing more systematic and structured languages.


find out that controlling the relative training speed dynamics enable to strongly control language emergent protocol properties.

%Populations have always been perceived as a structuring component for language to emerge and evolve: the larger the population, the more systematic the language. While this observation is widespread in the sociolinguistics literature, it has not been reproduced in computer simulations with deep reinforcement learning agents.
%In this paper, we thus aim to clarify this apparent contradiction. 
%We thoughtfully explore emergent language properties by varying agent population size in the speaker-listener Lewis Game. 
%After reproducing the experimental paradox, we challenge the simulation assumption that the agent community is homogeneous. To do so, we control the training speed or capacity of the agents by either asymetryzing the speaker-listeners properties or modifing each individuals within the population. 
%We show that introducing such heterogeneities naturally sort out the initial paradox for larger communities start developing more systematic and structured languages. %We then analyze other potential sources of heterogeneity and note how they may relate to the training speed, opening for further discussions in AI and sociolinguistics.  


==> buffer_file.tex <==





me and  However,  but does not explore the impact of the the size of population, and hypt. 
\bigbreak 
%
%
However,  
- peu de papier, resultats orienté
- focus on one hypothesis.
- 
il est difficile de bien decoreler les impacts de la p[opulation des autres facteurs d'entrainnement (comme le learning rate, les tailles des réseaux)]


In this paper, we







Among many environmental factors, population of individuals 

As a social environment parameter, population size has largely been studied in sociolinguistics. \mathieu{citations de la related} Evidences  demonstrate that larger populations develop less complex and more structured languages leading to a core assumption in emergent communication: one of the main limitation in emergent communication modeling is population scale. 



, through ethnographic~\citep{Lupyan2010}, experimental~\citep{Raviv2020a} or computationally simulated works~\citep{Levinson2012}.

 --  --  
%Languages vary in the ways they do in part due to different social environments in which they are learned and used. 





From a scientific perspective, understanding the conditions under which language evolves in communities of deep agents and its emergent features can shed light on human language evolution. From an applied perspective, endowing deep networks with the ability to solve problems interactively
by communicating with each other and with us should make them more flexible and useful
in everyday life. This article surveys representative recent language emergence studies from both of these two angles

language evolves in communities of
deep agents and its emergent features can shed light on human language evolution. 


When exploring language emergence, one must care about environment factors

Language emerge and it is structured by the environment.

What are the core component of language emergence

From a scientific
perspective, understanding the conditions under which language evolves in communities of
deep agents and its emergent features can shed light on human language evolution. From an
applied perspective, endowing deep networks with the ability to solve problems interactively
by communicating with each other and with us should make them more flexible and useful
in everyday life




Recent successes in deep learning are obtained with models that are passively exposed to massive amounts of text and/or images, and learn to rely on the statistical regularities they extracted from their training data.

The interactive, functional aspects of language and intelligence are completely ignored. To this extent, emergent communication aims at immersing models into \mathieu{complex} environments in order to improve models interactivity and hopefully language models. Most of environmental situations can be inspired by broader linguistics literature. 






Indeed, lots of ethnographic~\citep{Lupyan2010}, experimental~\citep{Raviv2020a} or computationally simulated~\citep{Levinson2012} results show that the emergence of language universals is tied to environmental pressures. It is mostly known as the \textit{Linguistic Niche Hypothesis}~\citep{niche-hypothesis}: languages may vary in the ways they do in part due to different social environments in which they are learned and used. 

As a social environment parameter, population size has largely been studied in sociolinguistics. \mathieu{citations de la related} Evidences  demonstrate that larger populations develop less complex and more structured languages leading to a core assumption in emergent communication: one of the main limitation in emergent communication modeling is population scale. 

In this paper, we study whether population size improve emergent languages in the context of a reconstruction game. 






% Studying language and population requires to dissociate two aspects of social environment: transmitting over generations (language evolution) and interacting in a community. The first has largely been studied in sociolinguistics \mathieu{(ref sur Kirby)} and show promising results for improving AI systems \mathieu{(papiers d'iterated learning)}. Based on ???, we study in this paper the second aspect.


==> old_comments.tex <==



% \mathieu{Paragraphe bonus}
% \paragraph{Learning asymmetry in emergent communication. } As part of this study, we will show that controlling speakers and listeners learning speed enables to control crucial language properties. Even though speakers and listeners tasks are different (reinforcement vs. supervision), task asymmetry has never been studied. All the more, most of emergent communication works are designed such that speakers and listeners have same parameters: same architecture, same network sizes, same learning rates, etc.~\citep{Lowe2020On, cao2018emergent,noukhovitch2021emergent}. When speakers and listeners are different, the asymmetry is not truly motivated.~\citep{evtimova2018emergent, chaabouni2019anti}


% \bigbreak 
% \mathieu{A METTRE EN DISCUSSION : en fait je pense qu'on complète graesser. Eux ils utilisent des agents qui ne se parle pas en parallèle. Avoir 3 agents => avoir un listener pivot. 2 agents, en parallèle, ça n'a pas de sens. Donc on peut dire qu'on confirme graesser et montre qu'il suffit d'avoir un agent pivot. On complète également boucharcourt 2019 qui étudient des agents qui ont un discours interne. Eux ont des dialogues internes, et à ce titre, peuvent obtenir un coordination. Du coup, ce n'est pas le nombre qui peut améliorer le résultat (comme il l'avance en discussion) mais le contrôle de la dynamic d'apprentissage.}

% \bigbreak 
% \mathieu{Inclure l'idée du spatio/temporelle}

% \bigbreak 
% \mathieu{A METTRE EN DISCUSSION : On peut relier nos résultats aux théories sur les second learners dans des populations + structure social du réseau.}
% .


% Population a plein d'effets.

% Understanding how and why linguistic structured emerged is a core question of language evolution. As of today, the emergence of linguistic structures is mainly explained by two theories. Firstly, Iterated Learning/cultural transmission \mathieu{blabla}. Secondly, a population based theory \mathieu{à reformuler} suggests that languages are highly linked to the social environment they emerge in. Indeed, historical studies have shown that different linguistic structures emerge in different societies depending on their size, network structure and the identity of their members \mathieu{réécrire ça}.

% The community size has particularly been studied in linguistic studies. It has been mainly argued that, on the one hand, community size is one of the most important drivers of natural languages evolution and, on the other hand, languages spoken in larger communities tend to be more structured (fewer and less elaborate morphological structures, simpler grammars) and more stable \mathieu{à vérifier les résultats de convergence et stabilité}. 

% Even if there are evidences of a correlation between community size and languages structures, no causal linked can be established based on raw linguistic data. Indeed, other environmental factors are highly correlated with community size: the connection sparsity in the social network, the geographic spread out of populations, the number of contact agents, the proportion of adult second learners. All of those factors provide alternative explanations and thus make it difficult to directly assign the emergence of language structures to community size.

% Contrarily to sociolinguistics researches that manage to infer theories from raw linguistic data, emergent communication provides tools to better control the characteristics of a population. Jusqu'à ce jour, les papiers ont principalement étudié les conditions d'émergence des universels du langages: compositionalité, généralisation, diversité ou encore efficacité (Zipf). On peut noter deux approches majoritaires dans la littérature: l'étude de biais inductif sur des systèmes de petites communautés d'agents, l'étude de la transmission culturelle (agent reseting et Iterated Learning). Si la seconde approche a parfois fait l'objet de l'étude de populations, la structure de la population ne fait pas l'objet d'une étude en tant que tel. 


% As of today, emergent communication have mainly studied small community systems mostly testing how Iterated Learning or inductive biases can help to recover language universals: compositionality, generalization or efficiency.

% \begin{enumerate}
%     \item \mathieu{Choi et al. : Ils ne s'intéressent pas spécifiquement aux populations mais suggèrent que un langage commun émerge quand on equip an agent with an innate mechanism that ties listening and speaking, such as the obverter technique, nor any explicit community-wide
%     coordination. }
%     \item \mathieu{Graesser et al. : Vrai étude de populations et d'aspects précis de sociolinguistique (avec $N_{speakers}=N_{listeners}$). Ils étudient principalement l'impact de l'introduction d'agents de contacts dans des populations d'agents. Leurs résultats portent principalement sur des questions de connections du réseau social (nombres d'agents de contacts wrt. la taille de la pop) et l'émergence d'un continuum linguistique. La taille de la population n'est pas étudiée en tant que tel mais apparait comme une CNS pour l'émergence d'un langage commun entre agents}
%     \item \mathieu{Bouchacourt et al.: jeu avec 2 agents (2 speakers + 2 listeners). Du point de vue population, étudie l'émergence d'un protocole symétrique (même langage). Result: single pairs of agents can't develop same language. Ils supposent qu'un protocole symmétrique peut émerger via l'augmentation de la community size (As convergence to a shared code is another basic property of human language, in future research we will explore ways to make it emerge.)}
%     \item \mathieu{Cogswell et al.: Ils simulent des populations avec des agents qui sont reset périodiquement (à la fois pop + cultural evolution). Ils focusent principalement sur la language evolution mais il y a un résultat (baseline) juste sur la population. Ils mentionnent le fait qu'avec la population il y a un certain gain de compo (ils citent en ref le papier de Rimor pour dire qu'on peut avoir un gain de compo sans cultural transmission), mais ce n'est pas très marqué. Rq. "As any Q-bot may be made to communicate with any A-bot, there is pressure for the population to adopt a unified language" ?}
%     \item \mathieu{Tieleman et al. : Ils étudient spécifiquement l'impact de la taille de la communauté sur la structure du language. Ils posent $N_{speakers}=N_{listeners}$. Ils ont des résultats préliminaires suggérant que les larges communautés développent des langages plus simples et structurés (tendent à conforter la littérature de socio-linguistique).}
%     \item \mathieu{Dagan et al.}
% \end{enumerate}



% Most of the characteristics of Referential games have been studied: impact of the input data structure, shape of the communication channel, architecture of the agents, design of the loss. However, one aspect of the setting is rarely mentioned: the impact of the task asymmetry on emergent languages properties. Most of the time, agents are designed with the same parameters or when it is not the case, it is not commented. Yet, Speaker and Listener tasks are very different, Speakers are often optimized with reinforcement learning procedures while Listeners are optimized with direct back-propagation. \textit{In this paper, we decided to address directly the issue of the task asymmetry between Speakers and Listeners and we show that the asymmetry learning \mathieu{speed} (which is dependent on all the parameters of the problem) has a tremendous impact on the property of the emergent languages.}

% \begin{enumerate}
%     \item \mathieu{spatial VS temporal regularization} 
%     \item \mathieu{Studies about population}
%     \item \mathieu{Experimental settings: broadcast VS. sampling}
%     \item \mathieu{core property: emergence of common language}
% \end{enumerate}

% \mathieu{\textbf{Transition:} Open question}









% \textbf{Confounding factor and Population Heterogeneity} Another thread of literature yet nuance those claims as it is challenging to certainly evaluate the influence of population size on language evolution~\citep{Nettle2012}. For instance, population-size and language evolution may be confounded with other factors such as: community wealth~\citep{nettle2000linguistic,mace1995latitudinal}, social structures~\citep{Trudgill2011,Lou-Magnuson2012} or number of contact agents~\citep{wray2007543}. Furthermore, multiple  works also discuss the importance of heterogeneity in shaping population properties~\citep{vaupel1979impact}, and already warned against homogeneous models of population

%In this paper, we highlight that the population size-effect may be more complex that first hypothesized. In our artificial setting, we show that community size effects only occur when unbalancing the number of speakers and listeners, latter suggesting the existence of an underlying key factor: learning speed asymmetry between speaking and listening.

%\paragraph{Confounding factors of population size.}
%Although  
%Another thread of literature yet nuance those claims as it is challenging to certainly evaluate the influence of population size on language evolution~\citep{Nettle2012}. For instance, population-size and language evolution may be confounded with other factors such as: community wealth~\citep{nettle2000linguistic,mace1995latitudinal}, local ecological resources~\citep{Nettle1996}, social structures~\citep{Trudgill2011,Lou-Magnuson2012}, number of contact agents~\citep{wray2007543} or existing  second-language learners~\citep{Winter2013,niche-hypothesis}. 
%In this paper, we highlight that the population size-effect may be more complex that first hypothesized. In our artificial setting, we show that community size effects only occur when unbalancing the number of speakers and listeners, latter suggesting the existence of an underlying key factor: learning speed asymmetry between speaking and listening.
%









% \subsection{Learning speed as an heterogeneity factor for agent modeling}
% \label{res:speed}

% As the communication task is co-adaptive, we cannot directly measure individual learning speed (speaker's training performances are dependent of listener's dynamics and vice versa). However, we can exhibit population inspired parameters that directly affect learning dynamics (\mathieu{show in appendix that is is the case)}:
% \begin{itemize}
%     \item Number of speakers $N_{s}$ (resp. listeners $N_{l}$) within the population. Easy to model in computer science, altering the number of speakers and listeners indirectly affect agents learning speed (\mathieu{justif}). However, it is not realistic as real individuals are both speakers and listeners motivating the introduction of a more plausible control parameter. 
%     \item Number of speakers training steps $N_{s/steps}$ (resp. listeners training steps $N_{l/steps}$) controlling how often an agent is optimized. With this factor, we directly accelerate or slow down agents' degree of learning and thus agents' learning speed. We use learning steps instead of learning rates in order to ease optimization and avoid extreme cases (too large or too small learning rates).
% \end{itemize}

% In this section, we study those control parameters at the speaker-listener level (assuming all speakers are identical and all listeners are identical) and show how it directly impacts language properties.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[scale=0.6]{figures_test/matrix2.png}
%     \caption{Matrix of emergent language entropies when varying the number of speakers and listeners within the population. Evolution of the entropy with the ratio of agents $\frac{N_{l}}{N_{s}}$}
%     \label{fig:hete1}
% \end{figure}

% \paragraph{Relative number of speakers and listeners within the population alter language properties.} 

% \begin{figure}[h!]
%     \centering
%     \includegraphics[scale=0.5]{figures_test/fig_rhos.png}
%     \caption{Evolution of emergent language properties as a function of $\rho_{step}$ and $\rho_{agents}$}
%     \label{fig:hete2}
% \end{figure}

% In Figure~\ref{fig:hete1} \mathieu{matrix}, we show how emergent languages entropy evolves when $N_{s}$ and $N_{l}$ vary in the populations. We can notice that the color gradient is stable  when the number of agents grows along the diagonal ( $N_{s}=N_{l}$) but that there are large entropy variations along the anti-diagonal. When $N_{s}$ is high and $N_{l}$ is low (bottom-left), populations develop high entropy languages; on the contrary, when $N_{s}$ is low and $N_{l}$ is high (top-right), agents develop almost deterministic languages. As the key factor is the relative number of speakers and listeners within the population, we then introduce $\rho_{agents}=\frac{N_{l}}{N_{s}}$: the ratio between the number of listeners and speakers. In Figure~\ref{fig:hete1} \mathieu{courbe}, we show that language entropy decreases with $\rho_{agents}$. In Figure~\ref{fig:hete2}, we show that $\rho_{agents}$ also impacts other language properties
% : speakers synchronization, compositionality and generalization increase with $\rho_{agents}$.

% \paragraph{Relative number of learning steps control language properties.} The same tendency is observed when varying the number of agents steps: the absolute values of $N_{s/steps}$ and $N_{l/steps}$ are not crucial, yet their relative number is. Indeed, we show in Figure~\ref{fig:hete2} that language properties evolve similarly with $\rho_{steps}:=\frac{N_{s}}{N_{l}}$ and $\rho_{agents}$ with the same extreme cases. 
% We can propose an interpretation of those extreme cases. When $\rho_{steps} \ll 1$, listeners have enough learning steps to learn speakers policies between each speaker update. Thus, as soon as speakers make their \{input,message\} mapping injective (ie. each message refers to a single input without ambiguity), the task is solved as listeners perfectly learn it. Hence, speakers do not have to adapt a lot and are close to their initial policy explaining why speakers' languages are not aligned, are highly entropic (speakers are initialized with random policies) and poorly compositional. On the contrary, when $\rho_{steps} \gg 1$, most of the co-adaptation work is performed by speakers. As speakers have lots of optimization steps before listeners evolve, they can finely estimate the reward landscapes and then target the messages that maximizes the joint distribution of listeners' rewards leading to low entropy policies. Because speakers all solve the same communication task~\footnote{actually the only requirement is the monotony between speakers' rewards}, they align on almost the same language. Eventually, we interpret the gain of compositionality to ease-of-learning~\citep{li2019ease}: speakers adopt more compositional languages as they are faster to learn for listeners. 

% \paragraph{Learning speed as structuring parameter for population modeling.} We have showed in the context of a 10 speakers-10 listeners population, that controlling agents learning speed (by indirectly controlling agents' rate of optimization steps) influences language properties with well defined extreme cases. In particular, emergent languages properties are highly dependent of the relative learning speed between agents. 
% Actually, we show in Appendix(\mathieu{one agent}) that results with $\rho_{steps}$ are independent of the number of agents meaning that $\rho_{ratio}$ can be used to alter emergent languages properties only with a single pair of agents.















%\paragraph{Understanding asymmetries effects.}
%We have demonstrated in Section \ref{res:speed} that learning asymmetry between speaker and listener (via optimization rate and agent capacity) controls emergent languages asymmetries. We can propose interpretations of the observed trends. 

%Let's first interpret the impact of $\rho_{speed}$. When $\rho_{speed} \ll 1$, i.e. $p_{s} \ll p_{l}$, the listener have enough learning steps to learn speakers' policies between each speaker update. Thus, as soon as speakers make their \{input,message\} mapping unambiguous, i.e. each message refers to a single input, the task is solved as listeners perfectly learn the mapping. Hence, speakers do not have to adapt a lot from their initial policy. As speakers are initialized with random policies, it then implies that speakers' languages are not aligned, are highly entropic and poorly compositional. On the contrary, when $\rho_{speed} \gg 1$, i.e. $p_{s} \gg p_{l}$, most of the co-adaptation work is performed by speakers. As speakers have lots of optimization steps before listeners evolve, they can finely estimate the reward landscapes and then target the few messages that maximize the distribution of listeners' rewards leading to low entropy policies. Because speakers all solve the same communication task, they align on almost the same language. Eventually, we interpret the gain of compositionality to "ease-of-learning"~\citep{li2019ease}: speakers adopt more compositional languages as they are faster to learn for listeners. We therefore discriminate two extreme cases:
%\begin{itemize}
%    \item Slow speaker/Fast listener: the speaker is the attractor, most of the co-adaptation is performed by the listener, and the emergent language is chaotic.
%    \item Fast speaker/slow listener: the listener is the attractor, most of the co-adaptation is performed by the speaker, and the emergent language is more coherent.
%\end{itemize}

%Second, $\rho_{capacity}$ is harder to interpret. Indeed, one could interpret the gain of compositionality and entropy to the limited capacity of the listener~\citep{resnick2019capacity}. However, we question this hypothesis as the absolute capacity of an agent is not key in our experiments (the upper bound of compositionality and lower bound of entropy is obtained with several hidden sizes from 8 to 128). Yet the ratio of capacities strongly influences the trend. We suggest that capacity effects may be a confounding effect of learning speed. In Appendix~\mathieu{S}, we actually show that a bigger agents co-adapt faster and slow down their partners. We therefore formulate the following hypothesis. the speaker and listener try to mutually estimate their models. Then, when the speaker (resp. listener) becomes larger, there is no learning limitations due to capacity and parameters can adapt quickly. Furthermore, it becomes harder for the listener (resp. speaker) to build a fine estimate of speaker's model (resp. listener's model) since it has a more complex model to estimate.
%Therefore, we argue that part of the effects observed with $\rho_{capacity}$ could also be explained by the relative learning speed between the speaker and listener.

%\paragraph{What are the mechanisms behind population effects ?} Through Section \ref{results}, we shed light on three population results: when population is homogeneous, no structure is promoted with the community size (1) ; when population is heterogeneous, increasing population size reduces language properties variance (2) and generally improves language properties (3). Let's now provide intuitions on the mechanisms behind those results.

%\mathieu{Détailler en ajoutant la notion de listener attracteur / listener neutre => bien dire qu'un listener lent c'est tjrs relativement au speaker}

%First, result (1) questions our naive expectations about populations. 
%\mathieu{mention below that we are working on small communities}
%First, result (1) questions our naive expectations about populations. From a first sight, we can think that increasing population size would force speakers to develop a unique, low entropy and structured language in order to suit every listeners. However, the main limitation of this assumption is that the game is co-adaptative. Indeed as soon as listeners are able to learn several, unstructured language, language structuring fails. We could totally imagine a situation where 1 speaker communicate with $N \gg 1$ listeners. If all listeners are "fast" enough to learn speaker's language, there is no real pressure applied on speaker toward structure. Then, we can think that increasing the number of agents entail agents to synchronize on a structure language because both the communication channel and listeners' capacities are limited. However, with realistic models, communication channel is very large enabling the emergence of many languages and listeners' model are able can also learn lots of languages. Merging those two reasons, we see that naively increasing community size of an homogeneous population is not constraining enough to explain the emergence of structured and systematic languages.

%increasing homogeneous population size implies that each speaker communicate with a lot of listeners requiring the generation of a general language. However, we suggest that the homogeneous population of listeners is almost equivalent to unique mean listener that defines a new - joint - distribution of reward. In other word, increasing population size is almost equivalent of fitting a new initialization of a bigger listener. Despite the model update, we are skeptical of the interest of such modeling. Then we would expect, the augmentation of the number of speakers to produce a kind of bottleneck effect that then could help structure and synchronize languages. However, with the architectures and number of agents consider, listeners are overparametrized and there is no chance of observing such bottleneck effect. We would suggest to either largely augment the community size or reduce the models to study such effect.

%Second, when working with heterogeneous populations, variance reduction is an expected effect. Indeed, when community is small, the average agent learning parameters are way more variable than for large communities. There is a fair probability of sampling small communities where learning parameters lead either structured or chaotic languages. On the contrary, when community becomes large learning speeds get accurately closer to the mean defined by the distribution leading to more systematic properties. 

%Third, the overall improvement of language properties is harder to characterize. Results of Section~\ref{res:speed} suggest that language properties are complex function of agents learning speed and especially of agents relative learning speed. In particular, language structuring is mostly driven by couples of fast speakers / slow listeners. It turns out that increasing population size promotes speakers and listeners from the distribution tails, that is, fast speakers and slow listeners. Therefore, we hypothesize that this is the promotion of such agents when $N$ becomes large that entails the population to structure languages. Indeed, slow listeners (relatively to speakers) attract languages into a unique, low entropy, compositional language. As a continuation of this work, it should be interesting to provide a quantitative framework of the impact of learning speed differences and evaluate whether language development could be seen as a dynamic system problem.




% \paragraph{Heterogeneity factors within populations.} 

% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{figures_test/capacity.png}
%     \caption{Evolution of language properties with $\rho_{capacity}$ \mathieu{ATTENTION figure avec un autre jeu de paramètres}}
%     \label{fig:capacity}
% \end{figure}

% In Section \ref{results}, we have chosen to use learning speed as heterogeneity factor, by indirectly control learning steps.
% This choice is motivated because most of potential control parameters we thought of before experiments actually indirectly affect learning speed. 

% As an example, we can consider another control parameter that seems to be very different to learning speed: LSTMs hidden sizes. When reproducing experiments of Section~\ref{res:speed} with a new ratio of speaker-listener capacities: $\rho_{capacity}:=\frac{h_{s}}{h_{s}}$ (where $h_{s}$ and $h_{l}$ is speaker and listener hidden sizes), we note exactly the same trend: the absolute hidden size of an agent has little impact on language properties (even for very small sizes $(h_{s},h_{l})=(8,8)$ pushing away a bottleneck hypothesis) but the relative speaker-listener sizes is crucial. Once again, we see that this parameter has to be considered in a relative way. We actually hypothesize that $\rho_{capacity}$ is a confounder of learning speed asymmetry between Speakers and listeners. In Appendix \mathieu{à faire}, we provide intuitions that bigger agents learn faster and are harder to adapt by the other agents.




% \section{Old Results}
% \label{oresults}

% \subsection{Questioning homogeneity in population design}.
% \label{res:homogeneity}



% \begin{figure}[h!]
%     \centering
%     \includegraphics[scale=0.55]{figures_test/fig_matrix.png}
%     \caption{Matrix}
%     \label{fig:my_label}
% \end{figure}

% As discussed in the introduction, we explore the impact of community size on language structures. We first test this hypothesis by naively increasing the community size of the homogeneous population $\mathcal{P}_{homogeneous}$ (\mathieu{définir dans la méthode}) where agents are identically designed. We increase populations in two ways. First, we extend population size setting $N_{s}=N_{l}$ as realistic agents are both speakers and listeners. Second, as the game is asymmetric, we also consider the case $N_{s} \neq N_{l}$ that can be helpful to understand the overall dynamics of the system. We store the results for entropy \mathieu{(choose metrics)} in Figure \mathieu{number}. 

% \paragraph{Increasing population sizes when agents are homogeneously designed does not structure languages}. As shown in Figure \mathieu{matrix}, increasing population size with $N_{s}=N_{l}$ has little impact on language entropy. In Figure \mathieu{diagonal}, we plot entropy values along the diagonal of the matrix ($N_{s}=N_{l}$). No clear dependency between entropy and population size can be observed. In Appendix \mathieu{other prop}, we extend this observation and show that other properties of emergent languages do not vary with community size (speaker synchronization, compositionality, generalization). We therefore confirm a trend of emergent communication literature: increasing community size has little impact on language properties when working with homogeneous populations. 

% \paragraph{Population size imbalance as a source of variation.} In Figure \mathieu{matrix}, if no major changes are observe along the diagonal ($N_{s}=N_{l}$), we see large variations of entropy as soon as $N_{s}$ and $N_{l}$ are unbalanced. In particular, when we look at the anti-diagonal in Figure \mathieu{anti-diagonal}, we note the emergence of either very low or very high entropy languages depending on $(N_{s},N_{l})$ balance. In particular: when $N_{s} \ll N_{l}$, agents develop low entropy languages ; when $N_{s} \gg N_{l}$, agents develop high entropy languages where almost all symbols are randomly distributed. Variations with $(N_{s},N_{l})$ balance are also observed on other language properties (see Appendix \mathieu{other properties}).

% \paragraph{Introducing heterogeneity into population design.} We interpret those variations by the learning asymmetry introduced by $N_{s}/N_{l}$ imbalance. Indeed, at each iteration of the game, a Speaker/Listener pair is sampled. When $N_{s}=N_{l}$, both speakers and listeners have the same probability to be sampled and thus to be optimized. Conversely, when the system is unbalanced, those sampling probabilities are different: $N_{s}$ and $N_{l}$ indirectly asymmetries speakers and listeners learning dynamics. 

% As these language variations are breaking homogeneity assumption (identical agent design, same number of speakers and listeners), we formulate the following hypothesis: Community size may be a structuring factor as soon as heterogeneity is introduced in population design. To test this hypothesis, we follow the subsequent protocol: in Section \ref{res:hete1} we first approach heterogeneity at the speaker/listener scale using $N_{s}/N_{l}$ imbalance factor as an inspiration to exhibit more plausible control parameters. Then, in Section \ref{res:hete2}, we distribute those parameters across the population and test whether community size affects emergent languages of heterogeneous populations.

% \subsection{Learning speed asymmetry controls emergent languages properties}.
% \label{res:hete1}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[scale=0.5]{figures_test/fig_rhos.png}
%     \caption{Rhos}
%     \label{fig:my_label}
% \end{figure}

% We first study how asymmetrizing speakers/listeners relative learning dynamics alters language properties. As shown in Section \ref{res:homogeneity}, the balance between $N_{s}$ and $N_{l}$ is such an asymmetry factor, yet not being relevant when modeling populations. Consequently, we introduce a new control parameter that mimics an analogous effect: $\rho_{steps}$. $\rho_{steps}$ is the ratio between the number of optimization steps of a speaker ($N_{s/steps}$) and a listener ($N_{l/steps}$). This parameter thus controls the relative degree of learning between the speakers and listeners without being directly dependent of population size. At each iteration, a speaker/listener pair is sampled and plays an instance of the game. Then the speaker (resp. listener) has a probability $\frac{N_{s/steps}}{\max(N_{s/steps},N_{l/steps})}$ (resp. $\frac{N_{l/steps}}{\max(N_{s/steps},N_{l/steps})}$)  to realize an optimization step. At the end of the game, each speaker has been optimized $\rho_{steps}:=\frac{N_{s/steps}}{N_{l/steps}}$ times more or less than each listener. As a baseline, we also introduce $\rho_{agents}:=\frac{N_{s}^{-1}}{N_{l}^{-1}}$ that controls the relative number of listeners and speakers within the population. \mathieu{notation confusing}

% \paragraph{$\rho_{steps}$ and $\rho_{agents}$ control language properties. } In Figure \mathieu{rho}, we plot the evolution of different language properties (entropy, topographic similarity, speaker synchronization) as functions of $\rho_{steps}$ and $\rho_{agents}$. Firstly, we note that these properties vary similarly when playing with $\rho_{steps}$ and $\rho_{agents}$. It enforces the assumption that $N_{s}/N_{l}$ unbalance effects are actually due to learning dynamics changes. Secondly, we note that both parameters display two very distinct regimes: when $\rho_{steps},\rho_{agents} \gg 1$ emergent languages develop interesting properties: speakers manage to synchronize on almost a single language (synchronization rate close to 1) that has a very low entropy (peaky policies) and compositional patterns. On the contrary, when $\rho_{steps},\rho_{agents} \ll 1$, each speaker develops its own language (synchronization rate close to random similarity rate) and all those languages are very entropic and poorly compositional. Hence, we manage to introduce a core parameter $\rho_{steps}$ - the relative degree of learning - that allows to control language properties. 

% \paragraph{Learning speed as an overall mechanism.} Extreme trends of Figure \mathieu{rho} can be interpreted with $\rho_{steps}$. When $\rho_{steps} \ll 1$, listeners have enough learning steps to learn speakers policies at each time. Thus, as soon as speakers make their \{input,message\} mapping injective (ie. each message refers to a single input without ambiguity), the task is solved as listeners have enough learning steps to learn this mapping. Hence, speakers do not have to adapt a lot their initial policy in order to succeed in the task explaining why speakers' languages are not aligned, are highly entropic (speakers are initialized with random policies) and poorly compositional. On the contrary, when $\rho_{steps} \gg 1$, most of the co-adaptation work is performed by speakers. As speakers have lots of optimization steps before listeners evolve, they can finely estimate the reward landscapes and then target the messages that maximises the joint distribution of listeners' rewards. As rewards are ordered~\footnote{we remind that we choose here a continuous reward}, Speakers adopt low entropy policies concentrated on the messages providing best rewards. Because speakers all solve the same communication task~\footnote{actually the only requirement is the monotony between speakers' rewards}, they align on almost the same language (high synchronization rate). Eventually, we interpret the gain of compositionality to ease-of-learning~\citep{li2019ease}: speakers adopt more compositional languages as they are faster to learn for listeners. 

% \mathieu{Transition difficile} We hypothesizes that $\rho_{steps}$ actually discretizes a more general mechanism: the learning speed asymmetry between speakers and listeners. 

% \paragraph{Heterogeneity between speakers and listeners is not sufficient to unveil the community size paradox.} We have just shown that introducing a learning speed heterogeneity between speakers and listeners significantly affects language properties. Nevertheless, no dependency to community size can be exhibited. We actually show in Appendix \mathieu{single} that this control parameter can be reduced to a single speaker/listener pair. Consequently, a second type of heterogeneity is required to observe community size effects: heterogeneity within the population of speakers (resp. listeners).

% \subsection{Community size alter language properties of heterogeneous populations}.
% \label{res:hete2}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[scale=0.5]{figures_test/fig_pop.png}
%     \caption{Population}
%     \label{fig:my_label}
% \end{figure}

% We have just seen in Section \ref{res:hete1} speakers and listeners relative learning speed (controlled with $\rho_{steps}$) influences language properties, yet not being dependent of the community  size. Let's now consider the introduction of heterogeneity within the set of speakers and listeners. In this section, we define a distribution $\mathcal{D}_{s}$ (resp. $\mathcal{D}_{l}$) of speakers (resp. listeners) probability of being optimized (see Appendix \mathieu{params} for description of the distributions). We build a population as followed. We choose a community size $N$ ($N=N_{s}=N_{l}$). Then, each speaker $s_{i}$ (resp. listener $l_{j}$) is assigned a probability $P_{s_{i}}$ (resp. $P_{l_{j}}$). Then, at each iteration of the game, we sample a random speaker/listener pair $(s_{i},l_{j})$ that plays the game. Then, with probability $P_{s_{i}}$ (resp. $P_{l_{j}}$), speaker $s_{i}$ (resp. $l_{j}$) is optimized. 

% \paragraph{Community size affects languages properties.} In Figure \mathieu{hete}, we show how emergent languages properties (entropy, compositionality, speaker synchronization, generalization) evolve with the community size. We can notice two main effects: first, the variance significantly decreases with community size. In particular, when communities are small, randomness allow the emergence of 

%\paragraph{} Based on previous observation, we see that breaking the full symmetry and homogeneity had a tremendous impact on emergent language properties. We thus ask the following questions: is the difference between deep emergent communication models and empirical evidences explained by population modeling ? Does 

% \begin{figure}[h!] 
%     \begin{subfigure}[t]{.19\textwidth}
%     \includegraphics[width=1.\linewidth,height=1.\linewidth]{figures/ent_f_Nagents.png}
%     %\label{fig:ent_f_splist}
%     %\caption{Entropy}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.19\textwidth}
%     \includegraphics[width=1.\linewidth,height=1.\linewidth]{}
%   % \caption{Robustness to noise attacks}
%   % \label{fig:noise_f_splist}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.19\textwidth}
%     \includegraphics[width=1.\linewidth,height=1.\linewidth]{figures/testacc_f_Nagents.png}
%     %\caption{Test accuracy}
%     %\label{fig:tacc_f_splist}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.19\textwidth}
%     \includegraphics[width=1.\linewidth,height=1.\linewidth]{figures/compo_f_Nagents.png}
%     %\caption{Topographic similarity}
%     %\label{fig:compo_f_splist}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.19\textwidth}
%     \includegraphics[width=1.\linewidth,height=1.\linewidth]{figures/sim_f_Nagents.png}
%     %\label{fig:sim_f_splist}
%     %\caption{Similarity between agents languages}
%     \end{subfigure}
%     %\caption{Emergent language evaluation properties as a function of the number of agents  ($N_{speakers}=N_{listeners}$)}
%     \label{fig:prop_f_Nagents}
% %\end{figure}

% %\begin{figure}[h!]
%     \begin{subfigure}[t]{.19\textwidth}
%     \includegraphics[width=1.\linewidth,height=1.\linewidth]{figures/ent_f_Nsplist.png}
%     %\label{fig:ent_f_splist}
%     %\caption{Entropy}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.19\textwidth}
%     \includegraphics[width=1.\linewidth,height=1.\linewidth]{}
%     %\caption{Robustness to noise attacks}
%     % \label{fig:noise_f_splist}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.19\textwidth}
%     \includegraphics[width=1.\linewidth,height=1.\linewidth]{figures/testacc_f_Nsplist.png}
%     %\caption{Test accuracy}
%     %\label{fig:tacc_f_splist}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.19\textwidth}
%     \includegraphics[width=1.\linewidth,height=1.\linewidth]{figures/compo_f_Nsplist.png}
%     %\caption{Topographic similarity}
%     %\label{fig:compo_f_splist}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.19\textwidth}
%     \includegraphics[width=1.\linewidth,height=1.\linewidth]{figures/sim_f_Nsplist.png}
%     %\label{fig:sim_f_splist}
%     %\caption{Similarity between agents languages}
%     \end{subfigure}
%     %\caption{Emergent language evaluation properties as a function of the ratio between the number of Speakers and the number of Listeners  ($\frac{N_{speakers}}{N_{listeners}}$)}
%     \label{fig:prop_f_splist}
% %\end{figure}

% %\begin{figure}[h!]
%     \begin{subfigure}[t]{.19\textwidth}
%     \includegraphics[width=1.\linewidth,height=1.\linewidth]{figures/ent_f_steps.png}
%     \label{fig:ent_f_steps}
%     \caption{Entropy}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.19\textwidth}
%     \includegraphics[width=1.\linewidth,height=1.\linewidth]{}
%     \caption{Robustness to noise}
%     \label{fig:noise_f_steps}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.19\textwidth}
%     \includegraphics[width=1.\linewidth,height=1.\linewidth]{figures/acc_f_steps.png}
%     \caption{Test accuracy}
%     \label{fig:tacc_f_steps}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.19\textwidth}
%     \includegraphics[width=1.\linewidth,height=1.\linewidth]{figures/compo_f_steps.png}
%     \caption{Topographic similarity}
%     \label{fig:compo_f_steps}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.19\textwidth}
%     \includegraphics[width=1.\linewidth,height=1.\linewidth]{}
%     %\label{fig:sim_f_splist}
%     \caption{Language Similarity  }
%     \end{subfigure}
    
%     \caption{Evolution of emergent language evaluation properties as a function of the ratio between Speaker learning steps and Listener learning steps ($\rho_{learning}$)}
%     \label{fig:prop_f_steps}
% \end{figure}

==> result_V1.tex <==
RESULTS V1
All the results shown in this section are obtained with the compositionality game. In Appendix \ref{appendix:res_gen}, we show that these results are robust to game protocol changes. \mathieu{maybe try to see if we can superpose the dots of both games on the same plots}.

\subsection{2 agents games: learning step ratio as a control parameter of  emergent languages entropy}

\mathieu{Problème global de discours. Est-ce que les propriétés de comm et de structure sont des conséquences de la chute d'entropie ou du learning ratio per se ? Je ne sais pas trop comment orienter le discours}

\mathieu{Peut-être orienter: structure (entropy+compo) et communication perf (gen+robustness)}

Firstly, we are going to analyze the evolution of emergent language properties as a function of the learning ratio between the Speaker and the Listener in a 2 agents game. As mentioned in Section \ref{method}, we control this learning ratio with the parameter $\rho_{learning}$ equal to the ratio between the number of Speaker learning steps during a training episode and the number of Listener learning steps during a training episode. In Figure \ref{fig:prop_f_steps}, we study a range of ratio $\rho_{learning}$ between $10^{-2}$ and $10^{2}$ (eg. $\rho_{learning}=10^{-2}$ means that Listener has 100 optimization steps in one episode while Speaker has 1 optimization step ; $\rho_{learning}=10^{2}$ means that Speaker has 100 optimization steps in one episode while Listener has 1 optimization step). One can note that when $\rho_{learning}$ is very low, Listener is almost optimal for every Speaker's optimization step (left part of the plots) ; when $\rho_{learning}$ is very high, Speaker is almost optimal for every Listener's optimization step (right part of the plots).

\begin{figure}[h!]
    \begin{subfigure}[t]{.24\textwidth}
    \includegraphics[width=1.\linewidth,height=1.\linewidth]{figures/ent_f_steps.png}
    \label{fig:ent_f_steps}
    \caption{Entropy}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.24\textwidth}
    \includegraphics[width=1.\linewidth,height=1.\linewidth]{}
    \caption{Robustness to noise}
    \label{fig:noise_f_steps}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.24\textwidth}
    \includegraphics[width=1.\linewidth,height=1.\linewidth]{figures/acc_f_steps.png}
    \caption{Evolution of the test accuracy}
    \label{fig:tacc_f_steps}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.24\textwidth}
    \includegraphics[width=1.\linewidth,height=1.\linewidth]{figures/compo_f_steps.png}
    \caption{Evolution of the topographic similarity}
    \label{fig:compo_f_steps}
    \end{subfigure}
    
    \caption{Evolution of emergent language evaluation properties as a function of the ratio between Speaker learning steps and Listener learning steps ($\rho_{learning}$)}
    \label{fig:prop_f_steps}
\end{figure}

\paragraph{Entropy is a decreasing function of learning step ratio} Figure \ref{fig:ent_f_steps} \mathieu{(pb de subref)} shows the evolution of the average entropy per symbol of emergent languages obtained for couple of agents trained with a given learning ratio $\rho_{learning}$. We can note a continuous evolution of the entropy between two extreme cases: when $\rho_{learning}$ is low (Listener optimal with respect to the Speaker), agents converge to emergent languages with high entropy \mathieu{(mention here the maximal value we can get)}. It means that the Speaker can use a large number of messages to refer to a given input $x$ (lots of synonyms). On the contrary, when $\rho_{learning}$ is high (Speaker optimal with respect to the Listener), agents converge to a language of very low entropy meaning that the Speaker almost send a unique message per input $x$ of the input space $\mathcal{X}$. 

We can interpret this result by characterizing the task of the Speaker and Listener. Speaker's task (characterized by a given learning speed $v_{speaker}$) is to find the messages that provide the best reward via sampling estimation. Listener's task (characterized by a given learning speed $v_{listener}$) is to learn as many messages sent by the Speaker as possible by mapping them to the correct input. The reward then control the rate of Listener's learning. The left side of the curve represents the case for which Listener's is almost optimal with respect to Speaker. Due to random initialization, Speaker starts with flat message distributions. Then, Speaker is slow enough to leave time for the Listener to learn a lot of synonyms (different messages referring to the same input). It means that a lot of messages get an (almost) optimal reward. Therefore, it is equivalent (in term of reward) for the Speaker to use one of those synonyms, leading to language with high entropy. On the contrary, when Speaker is almost optimal with respect to Listener, Speaker has always an optimal estimation of the reward landscape defined by the Listener. Right from the beginning of the training, Speaker can therefore target the small set of messages that provide the best rewards. Meanwhile, Listener has not time enough to learn a lot of synonyms (before Speaker focus of a small number of words). Consequently, Speaker converges toward a language with very low entropy (almost a 1:1 mapping between the inputs and messages).

\mathieu{Mention that a minimal co-adaptation is required}

\paragraph{Low entropy languages have better communication properties} Previous paragraph shows that the learning ratio is a control parameter of the final entropy of the emergent language. However, we can wonder whether entropy is linked to other communication properties. In Figure \ref{fig:tacc_f_steps} and \ref{fig:noise_f_steps}, we see that languages with low entropy are also those that better generalize (better accuracies on test set) and that are more robust to noise attacks on the latent space. It means that low entropy languages are redundant: the gain of fixed symbols compared to high entropy languages provide information and are not kind of noise symbols.  \mathieu{clarifier}

\paragraph{Low entropy languages are more structured} Additionaly, Figure \ref{fig:compo_f_steps} shows that low entropy languages are also more structured. Indeed,  when Speaker is almost optimal at every listener's optimization step, emergent languages reach high topographic similarity values meaning that the language is compositional. \mathieu{develop}
\mathieu{(mention here the bounds of typical top sim values)}.
\mathieu{here question the topsim. Maybe high entropy languages are also structured over the symbols with low entropy.}

\paragraph{Actually, all the parameters of the problem influence the ratio of learning speeds} In this Section, we have introduce a control parameter: the learning ratio $\rho_{learning}$ that allow to control the degree of learning between the Speaker and the Listener, and indirectly simulate experiments in which both agents have different learning speeds. However, it has to be mentioned that actually all the parameters of the game have an impact on the learning speed. In Appendix \ref{appendix:parameters_asym}, we show that playing with either the size of the agents (and thus the complexity of the policy models) or the learning rate allow us to obtain exactly the same tendencies. Consequently, it is important to be aware that in a co-adaptation communication game, the choice of parameters has a direct impact on the structure of the emergent languages. \mathieu{rendre le truc positif par rapport à la contrib + rendre plus fluent l'idée d'asymmétrie de vitesse}

\subsection{Population games: playing with the number of speakers and listeners is equivalent to playing the the learning steps}

\mathieu{Transition (peut-être à déplacer dans la méthode)}. As we have just seen the previous Section, the degree of asymmetry between agents' learning speed (that can be controlled via $\rho_{learning}$), has a direct impact on the entropy and communication properties of emergent languages. However, it is generally admitted \mathieu{(ajouter des ref)} that those properties (structure, generalization, robustness to noise) are obtained when dealing with sufficiently large communities of agents. In this Section, we are going to show that the crucial factor is not the total number of agents but rather the ratio between the number of speakers and listeners. Via a short analysis, we are going to hypothesis that the phenomenon at play is once again an asymmetry of learning speed rather than a population effect.

\begin{figure}[h!]
    \begin{subfigure}[t]{.19\textwidth}
    \includegraphics[width=1.\linewidth,height=1.\linewidth]{figures/ent_f_Nsplist.png}
    \label{fig:ent_f_splist}
    \caption{Evolution of the entropy}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.19\textwidth}
    \includegraphics[width=1.\linewidth,height=1.\linewidth]{figures/sim_f_Nsplist.png}
    \label{fig:sim_f_splist}
    \caption{Evolution of the similarity between agents languages}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.19\textwidth}
    \includegraphics[width=1.\linewidth,height=1.\linewidth]{}
    \caption{Evolution of the robustness to noise attacks}
    \label{fig:noise_f_splist}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.19\textwidth}
    \includegraphics[width=1.\linewidth,height=1.\linewidth]{figures/testacc_f_Nsplist.png}
    \caption{Evolution of the test accuracy}
    \label{fig:tacc_f_splist}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.19\textwidth}
    \includegraphics[width=1.\linewidth,height=1.\linewidth]{figures/compo_f_Nsplist.png}
    \caption{Evolution of the topographic similarity}
    \label{fig:compo_f_splist}
    \end{subfigure}
    \caption{Evolution of emergent language evaluation properties as a function of the ratio between the number of Speakers and the number of Listeners  ($\frac{N_{speakers}}{N_{listeners}}$)}
    \label{fig:prop_f_splist}
\end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=1.\linewidth,height=0.15\textheight]{figures/all_f_Nsplist.png}
%     \caption{Evolution of emergent language evaluation properties as a function of the ratio between the number of Listeners and the number of speakers ($\frac{N_{listeners}}{N_{speakers}}$) \textbf{passer en a/b/c}}
%     \label{fig:ent_f_steps}
% \end{figure}

\paragraph{The size of the community is not the key factor explaining the emergence of structural and \textit{generalization} properties} \mathieu{IL FAUT UN PLOT EXPLICATIF EN PLUS (appendix ?) qui montre que le nombre absolu d'agents n'est pas le facteur clef).} As shown in \mathieu{(???)}, the communication properties are not significantly influenced by the total number of agents (in this experiment we set $N_{speakers}=N_{listeners}$). In particular, \mathieu{(il faut ajouter un plot pour fix number of speakers and listeners.)} when fixing the number of agents of one type (resp. speakers and listeners) and playing with the number of agents of the other type (resp. listeners and speakers) has not the same effect. Increasing $N_{listeners}$ when $N_{speakers}$ is fixed tend to improve emergent languages structures (lower entropy, better compositionality) and communication performances (better robustness to noise and accuracy on the test set). On the contrary increasing $N_{speakers}$ when $N_{listeners}$ is fixed tend to produce emergent languages with poorer structures (higher entropy, worse compositionality) and worse communication performances (worse robustness to noise and accuracy on the test set). Therefore, the decisive factor at play seems to be the ratio between the number of speakers and the number of listeners rather than the absolute number of agents.

\paragraph{Communication properties are improved when $\frac{N_{speakers}}{N_{listeners}}$ is increasing} Figure \ref{fig:ent_f_splist}, \ref{fig:noise_f_splist}, \ref{fig:tacc_f_splist} and \ref{fig:compo_f_splist} display respectively the evolution of the entropy, robustness to noise attacks, accuracy of test set and compositionality as functions of the ratio between the number of speakers and listeners. As we can see, all the communication properties are improved when $\frac{N_{listeners}}{N_{speakers}}$ is increasing. It means that the relative number of speakers and listeners is a key factor influencing communication properties, rather than the absolute number of agents \mathieu{à reformuler}.

Additionally, we study another property that is specific to populations: the similarity between Speaker's languages. As shown in Figure \ref{fig:sim_f_splist}, average similarity between Speaker's languages increase when $\frac{N_{speakers}}{N_{listeners}}$ is increasing. It means that for a fixed number of speakers, the more Listeners they are in the population, the more synchronized Speaker's languages. 

\paragraph{$\frac{N_{speakers}}{N_{listeners}}$ and $\rho_{learning}$ are similar control parameters of communication properties} We can observe that the trends are the same when playing with $\frac{N_{listeners}}{N_{speakers}}$ in the population game and with $\rho_{learning}=\frac{N_{steps/speaker}}{N_{steps/listener}}$ in the 2 agent game. Actually, it is not a surprise: when optimizing the system by sampling pairs of speaker-listener at each step, the number of speakers and listeners indirectly control the ratio of learning steps between speakers and listeners. Indeed, at each optimization step, each speaker (resp. listener) has a probability $\frac{1}{N_{speakers}}$ (resp. $\frac{1}{N_{listeners}}$) to be selected. Therefore, each speaker is optimized $\frac{N_{listeners}}{N_{speakers}}$ more or less than each listener, parameter close to our definition of  $\rho_{learning}$. 

From a broader point of view, it means that what has been considered as a population effect could actually be the result of an asymmetry of learning speed and a consequence of the sampling protocol \mathieu{à reformuler, peut-être introduire ici le speaker/listener moyen}. In Appendix \mathieu{(?)}, we actually show that when considering broadcasting situations (speaker speaking to several listeners at the same time), ... \mathieu{préparer le plot du broadcasting et ses résultats et reformuler l'explication en fonction}.

\paragraph{$\frac{N_{speakers}}{N_{listeners}}$ and $\rho_{learning}$ as complementary factors} As we have just seen, the ratio between the number of Listeners and Speakers and the ratio of learning steps between Speakers and Listeners have an analogous impact on communication properties. Actually, both of those parameters can be used at the same time. As an example, let's consider the case of a population of two speakers and one listener. \mathieu{appendix ou figure}. By assumption $\frac{N_{listeners}}{N_{speakers}}=2$ such that we expect agents to have a similarity close to $0.7$. However, we can show that using $\rho_{learning}$, we can either make agents converge toward a unique similar language or 2 very distinct ones. In the end, $\frac{N_{speakers}}{N_{listeners}}$ and $\rho_{learning}$ behave as complementary factors that control the properties of emergent languages.
